Deep Learning Based Channel Estimation in High Mobility Communications Using Bi-RNN Networks

Doubly-selective channel estimation represents a key element in ensuring communication reliability in wireless systems. Due to the impact of multi-path propagation and Doppler interference in dynamic environments, doubly-selective channel estimation becomes challenging. Conventional channel estimation schemes encounter performance degradation in high mobility scenarios due to the usage of limited training pilots. Recently, deep learning (DL) has been utilized for doubly-selective channel estimation, where convolutional neural network (CNN) networks are employed in the frame-by-frame (FBF) channel estimation. However, CNN-based estimators require high complexity, making them impractical in real-case scenarios. For this purpose, we overcome this issue by proposing an optimized and robust bi-directional recurrent neural network (Bi-RNN) based channel estimator to accurately estimate the doubly-selective channel, especially in high mobility scenarios. The proposed estimator is based on performing end-to-end interpolation using gated recurrent unit (GRU) unit. Extensive numerical experiments demonstrate that the developed Bi-GRU estimator significantly outperforms the recently proposed CNN-based estimators in different mobility scenarios, while substantially reducing the overall computational complexity.

==> 4soa_cnn_estimators.tex <==
\section{SoA DL-based Channel Estimation} 
\label{literature_review}

In~\cite{WI-CNN} a {\ac{CNN}} aided {\ac{WI}} channel estimation schemes have been proposed. The WI-CNN estimators use adaptive frame structure according to the mobility scenario. The idea is to avoid using comb pilot allocation and insert $Q$ pilot {\ac{OFDM}} symbols with different configuration within the transmitted {\ac{OFDM}} frame instead. 
%This frame structure was proposed motivated by the fact the vehicle velocity is a known parameter that can be exchanged between all vehicular network nodes. 
In this context, the \ac{WI}-{\ac{CNN}} estimators employ one, two, and three pilot symbols in low, high, and very high mobility scenarios, respectively. Moreover, two pilot allocation schemes are used for the inserted pilot symbols, such that: (\textit{i}) Full pilot allocation ($\text{FP}$): where $K_\text{on}$ pilots are inserted within each pilot symbol. (\textit{ii}) $L$ pilot allocation ($\text{LP}$): this allocation is motivated by the fact only $L$ pilots are enough to estimate the channel impulse response. Following the selection of the frame structure and the pilot allocation scheme, the \ac{WI}-{\ac{CNN}} estimators proceed as follows 

%
\begin{itemize}
 %   
    \item \textbf{Pilot symbols channel estimation}: In order to estimate the channel at the inserted pilot symbols, the basic {\ac{LS}} denoted as \emph{{\ac{SLS}}} estimation is applied using the received preambles as shown in~\eqref{eq: LS}, and using each received pilot symbol such that
        \begin{equation}
        \hat{\tilde{\ma{h}}}_{{\text{SLS}}_{q}}[k] = \frac{\tilde{\ma{y}}^{(p)}_{q}[k]}{\tilde{\ma{p}}[k]} = \tilde{\ma{h}}_q[k] + \tilde{\ma{v}}_{{q}}[k], ~ k \in \Kon.
        \label{eq: SLSP}
        \end{equation}
%        
        $\tilde{\ma{v}}_{q}[k]$ represents the noise at the $q$-th received pilot symbol and
        $\tilde{\ma{Y}}_{Q} = [\tilde{\ma{y}}^{(p)}_{1}, \dots,  \tilde{\ma{y}}^{(p)}_{q}, \dots, \tilde{\ma{y}}^{(p)}_{Q}] \in \compl ^{K_{\text{on}}\times Q}$. $q$ denotes the inserted pilot symbol index, where $1 \leq q \leq Q$.
        On the other hand, the  \emph{{\ac{ALS}}} relies on the fact that $\tilde{\ma{h}}_{{q}} =\ma{F}_{\text{on}} {\ma{h}}_{q,L}$, where ${\ma{h}}_{q,L} \in \compl ^{L\times 1}$ denotes the channel impulse response at the $q$-th received pilot symbol that can be estimated as follows
        \begin{equation}
        %\begin{split}
        \hat{\ma{h}}_{q,L} = \ma{F}_{\text{on}}^{\dagger} \hat{\tilde{\ma{h}}}_{{\text{LS}}_{q}},~  k \in \Kon,
        %\end{split}
        \label{eq:ALS1}
        \end{equation}
 %       
        where $\ma{F}_{\text{on}}^{\dagger} = [(\ma{F}_{\text{on}}^{\text{H}} \ma{F}_{\text{on}})^{-1} \ma{F}_{\text{on}}^{\text{H}}]$ is the pseudo inverse of the scaled DFT matrix $\ma{F}_{\text{on}} \in \compl^{K_{\text{on}} \times L}$. After that, the accurate {\ac{LS}} estimation can be obtained by applying the {\ac{DFT}} interpolation of $\hat{\ma{h}}_{q,L}$ as follows
        \begin{equation}
        %\begin{split}
        \hat{\tilde{\ma{h}}}_{{\text{ALS}}_{q}} = \ma{F}_{\text{on}} \hat{\ma{h}}_{q,L},  ~ k \in \Kon.
        %\end{split}
        \label{eq:ALSP}
        \end{equation}
         
         We note that the \emph{{\ac{ALS}}} and \emph{{\ac{SLS}}} are used for FP allocation, whereas, for LP allocation the channel estimation requires only $L$ pilots in each pilot symbol, and can be computed as follows
    \begin{equation}
 %   \begin{split}
    \hat{\ma{h}}_{q,L} = \ma{F}_{p}^{\dagger} \hat{\tilde{\ma{h}}}_{{\text{LS}}_{q}},~  k \in \Kp.
%    \end{split}
    \label{eq:dft4}
    \end{equation}
%
    $\hat{\tilde{\ma{h}}}_{\text{LS}_{q}}$ here represents the {\ac{LS}} estimated channel for the $q$-th pilot symbol at the $L$ equally spaced inserted pilot subcarriers, where $K_{p} = L$ and $\ma{F}_{p}^{\dagger} = [(\ma{F}_{p}^{\text{H}} \ma{F}_{p})^{-1} \ma{F}_{p}^{\text{H}}]$ is the pseudo inverse matrix of $\ma{F}_{p} \in \compl^{K_{\text{p}} \times L}$. After that, {\ac{DFT}} interpolation based estimation can be used employing $\hat{\ma{h}}_{q,L}$ to estimate the channel for the $q$-th pilot symbol as follows
%         
    \begin{eqnarray}
    \hat{\tilde{\ma{h}}}_{\text{DFT}_{q}} = \ma{F}_{\text{on}} \hat{\ma{h}}_{q,L},  ~ k \in \Kon.
    \label{eq:dft5}
    \end{eqnarray}

    \item \textbf{Data symbols channel estimation}: After estimating the channel at the inserted $Q$ pilot symbols, the WI-CNN estimator divides the received frame into several sub frames that are grouped as follows
    
    \begin{equation}
          \hat{\tilde{\ma{H}}}_{q} = [\hat{\tilde{\ma{h}}}_{q-1}, \hat{\tilde{\ma{h}}}_{q}],~ q = 1, \cdots Q.
      \end{equation}
      
      We note that $\hat{\tilde{\ma{h}}}_{0} = \hat{\tilde{\ma{h}}}_{\text{LTS}}$ and $\hat{\tilde{\ma{h}}}_{q}$ refers to the implemented {\ac{LS}} estimation according to the utilized pilot allocation scheme. After that, the estimated channel for the $i$-th received data {\ac{OFDM}} symbol within each sub-frame is calculated as a weighted summation of the estimated channels at the pilot symbols, such that 
      
      \begin{equation}
          \hat{\tilde{\ma{H}}}_{{\text{WI}}_{f}} =  \hat{\tilde{\ma{H}}}_{{f}} \ma{C}_{f}
      \label{eq:WI_LS}
      \end{equation}
      where $\hat{\tilde{\ma{H}}}_{f} \in \compl^{ K_{\text{on}} \times 2} $ denotes {\ac{LS}} estimated channels at the pilot symbols within the $f$-th sub-frame. $\ma{C}_{f} \in \mathbb{R}^{2 \times I_{f}}$ denotes the interpolation weights of the $I_{f}$ {\ac{OFDM}} data symbols within the $f$-th sub-frame. $\ma{C}_{f}$ interpolation weights are calculated by minimizing the {\ac{MSE}} between the ideal channel $\tilde{\ma{H}}_{{f}}$, and the {\ac{LS}} estimated channel at the {\ac{OFDM}} pilot symbols $\hat{\tilde{\ma{H}}}_{{f}}$ as derived in~\cite{ref_interpolation_matrix}. 
    
    
       
    \item \textbf{CNN Post processing}: According to the analysis performed in~\cite{WI-CNN}, an optimized {\ac{SR-CNN}} is employed on top of the {\ac{WI}} estimators in a low mobility scenario, whereas an optimized {\ac{DN-CNN}} is considered in high mobility one.    
    
    
\end{itemize}

The {\ac{WI}}-{\ac{CNN}} estimators suffer from high computational complexity, moreover, using noise alleviation {\acp{CNN}} is not sufficient to accurately estimate the doubly-selective channel. Therefore, we propose a {\ac{Bi}}-{\ac{GRU}} channel estimator that perform 2D interpolation, unlike the {\ac{SR-CNN}} and {\ac{DN-CNN}} networks which are based on noise alleviation techniques. Therefore, performance superiority of the proposed {\ac{Bi}}-{\ac{GRU}} channel estimator can be achieved while recording a significant computational complexity decrease in comparison to the {\ac{WI}}-{\ac{CNN}} estimators as illustrated in Section~\ref{simulation_results}.


  
 



==> 8acknowledgment.tex <==
\section*{Acknowledgment}
Authors acknowledge the CY Initiative of Excellence for the support of the project through the ASIA Chair of Excellence Grant (PIA/ANR-16-IDEX-0008).
